Feature2Vec: Distributional semantic modelling of human property knowledge

Feature norm datasets of human conceptual knowledge, collected in surveys of human volunteers, yield highly interpretable models of word meaning and play an important role in neurolinguistic research on semantic cognition. However, these datasets are limited in size due to practical obstacles associated with exhaustively listing properties for a large number of words. In contrast, the development of distributional modelling techniques and the availability of vast text corpora have allowed researchers to construct effective vector space models of word meaning over large lexicons. However, this comes at the cost of interpretable, human-like information about word meaning. We propose a method for mapping human property knowledge onto a distributional semantic space, which adapts the word2vec architecture to the task of modelling concept features. Our approach gives a measure of concept and feature affinity in a single semantic space, which makes for easy and efficient ranking of candidate human-derived semantic properties for arbitrary words. We compare our model with a previous approach, and show that it performs better on several evaluation tasks. Finally, we discuss how our method could be used to develop efficient sampling techniques to extend existing feature norm datasets in a reliable way.

==> old_table3.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccc}
\hline

\textbf{Concepts}            & \textbf{Properties}            \\ 
\iffalse
\underline{\textbf{Axe}}                         & \begin{tabular}{}  
\underline{\textbf{made\_of\_wood}} \,
\underline{\textbf{is\_sharp}} \,
\underline{\textbf{made\_of\_metal}} \,
\underline{\textbf{does\_cut}} \,
\underline{\textbf{has\_a\_handle\_handles}} \\
\underline{\textbf{has\_a\_blade\_blades}} \,
\underline{\textbf{is\_dangerous}} \,
\underline{\textbf{is\_a\_weapon}} \,
is\_long \\
\underline{\textbf{is\_a\_tool}}
\end{tabular} \fi                   \hline
\multirow{3}{*}{Kingfisher} & \multirow{3}{*}{\begin{tabular}{}
\underline{\textbf{has\_wings}} \,
\underline{\textbf{does\_fly}} \,
\underline{\textbf{has\_a\_beak}} \,
\underline{\textbf{has\_feathers}} \,
\underline{\textbf{is\_a\_bird}} \\
\underline{\textbf{does\_eat}} \,
has\_a\_tail \,
does\_swim \,
\underline{\textbf{has\_legs}} \,
does\_lay\_eggs \\ 
\end{tabular}} \\
                            &                       \\
                            &                       \\ \hline
\multirow{3}{*}{Avocado}    & \multirow{3}{*}{\begin{tabular}{}
\underline{\textbf{is\_eaten\_edible}} \,
\underline{\textbf{is\_tasty}} \,
\underline{\textbf{does\_grow}} \,
\underline{\textbf{is\_green}} \,
\underline{\textbf{is\_healthy}} \,
is\_used\_in\_cooking \\
\underline{\textbf{has\_skin\_peel}} \,
is\_red \,
is\_food \,
\underline{\textbf{is\_a\_vegetable}} \,
\end{tabular}} \\
                            &                       \\
                            &                       \\ \hline
\multirow{3}{*}{Door}                        &  \multirow{3}{*}{\begin{tabular}{} 
made\_of\_metal  \,
has\_a\_door\_doors \, 
is\_useful  \,
has\_a\_handle\_handles  \,
made\_of\_wood  \\
made\_of\_plastic  \,
is\_heavy  \,
is\_furniture  \,
does\_contain\_hold \,
is\_found\_in\_kitchens  \,
\end{tabular}}                   \\ 
                            &                       \\
                            &                       \\ \hline
                            
                          \begin{tabular}{}  Dragon  \end{tabular}                       &  \begin{tabular}{} 
is\_big\_large  \,
is\_an\_animal  \, 
has\_a\_tail  \, 
does\_eat  \,
is\_dangerous  \\
has\_legs \, 
has\_claws  \,
is\_grey  \,
is\_small  \,
does\_fly  \,
\end{tabular}             \\ \hline 
\end{tabular}
}

\caption{Top 10 predictions from CSLB-trained Feature2Vec model. The properties in bold and underlined are those that agree with the available ground truth features from the CSLB dataset. The first two concepts are from the CSLB test set, whilst the final two words were randomly sampled from the word embedding lexicon.}
\label{featpreds}
\end{table*}
